Listen, Look and Deliberate: Visual context-aware speech recognition using pre-trained text-video representations

In this study, we try to address the problem of leveraging visual signals to improve Automatic Speech Recognition (ASR), also known as visual context-aware ASR (VC-ASR). We explore novel VC-ASR approaches to leverage video and text representations extracted by a self-supervised pre-trained text-video embedding model. Firstly, we propose a multi-stream attention architecture to leverage signals from both audio and video modalities. This architecture consists of separate encoders for the two modalities and a single decoder that attends over them. We show that this architecture is better than fusing modalities at the signal level. Additionally, we also explore leveraging the visual information in a second pass model, which has also been referred to as a `deliberation model'. The deliberation model accepts audio representations and text hypotheses from the first pass ASR and combines them with a visual stream for an improved visual context-aware recognition. The proposed deliberation scheme can work on top of any well trained ASR and also enabled us to leverage the pre-trained text model to ground the hypotheses with the visual features. Our experiments on HOW2 dataset show that multi-stream and deliberation architectures are very effective at the VC-ASR task. We evaluate the proposed models for two scenarios; clean audio stream and distorted audio in which we mask out some specific words in the audio. The deliberation model outperforms the multi-stream model and achieves a relative WER improvement of 6% and 8.7% for the clean and masked data, respectively, compared to an audio-only model. The deliberation model also improves recovering the masked words by 59% relative.

==> Rebuttal.tex <==
We would like to thank you for your valuable time spent reviewing our paper and your thoughtful comments. Below, we address all comments and answer all questions point by point. The original reviewer comments are quoted (specified by quotation mark) which are followed by our responses starting with “*Response*”.



     **************************************      Reviewer 0C1E  ********************
     

"Novelty/Originality & Experimental Validation" : “Novel models are claimed but not convincingly.” and “The proposed multi-stream model looks similar to previous works that compare features with early and late fusion. In addition, the results could have included more baselines. Some within the literature of VC-ASR and some others for example in the area of caption generation. A stronger and clearer comparison of recognisers would have made the paper's claims more compelling.”

*Response*: We respectfully disagree with these statements. To address them, we first clarify the novelties of this study, then we will describe the possible baselines one would have for this study and why we chose the current ones.

Compared to the previous works, this study is novel in three aspects.  1) as opposed to all the previous studies for VC-ASR that used a fixed vector to represent the entire video, we leverage the visual context in the form of a sequence of features to represent objects, actions, and scenes that emerge at different time steps of a video. 2) Given the weak and noisy correlation between the transcriptions and the visual features for HOW2 data, we proposed a multi-stream model with a gating mechanism to fuse the input streams at each time step. We demonstrated that the gating mechanism is crucial to flexibly change the contribution of input streams where one modality is distorted. 3) most importantly, we proposed to leverage the visual information in a deliberation step on top of an audio-only model. In the proposed deliberation model, we leveraged a pre-trained text model to ground the hypothesis of the first decoder to the visual features to refine them and generate higher quality outputs. We showed that the deliberation model outperforms the baseline and multi-stream approaches and achieves a new state of the art VC-ASR performance for the HOW2 dataset.  In addition to the superiority in performance, as also pointed out by reviewer “0FE6”, the proposed deliberation model opens up an opportunity to refine the N-best hypotheses generated by existing pre-trained audio-only models by flexibly leveraging the visual context, if available. 
 

 
Regarding the baselines of this study, all the previous works for the VC-ASR task have used the HOW2 dataset to train and evaluate their systems. In the previous studies, as discussed in the introduction section of our paper, many of image-captioning inspired approaches such as initializing the decoder, or early decoder fusion have been investigated for VC-ASR task. For decoder initialization, they averaged pool the visual features to a fixed vector, then used this vector to initialize the decoder, or used it instead of the beginning of sentence (<bos>) token.  For the early decoder fusion, they also used a fixed vector to represent the visual context and concatenated this vector to all audio embedding vectors before being passed to the decoder.  However, we hypothesized that distilling the visual context into a fixed vector is not an effective approach, and we designed a multi-stream attention-based model with a gating mechanism to provide a more detailed and correlated visual context at each time step. We have also conducted experiments, not reported in the paper, examining the performance of the aforementioned baseline approaches, however, both early decoder fusion and decoder initialization underperformed our audio-only model (they hurt the performance rather than improving it). We will include these experiments in the camera-ready paper. It has also been demonstrated in [1] that for the HOW2 dataset, normalizing the audio features using the visual context outperforms initialization-based approaches. Therefore, for the baselines of this study, we compare the performance of our proposed models with a decent audio-only model and the normalization approach which had achieved the state of the art performance for VC-ASR task on HOW2 dataset [1]. 





  




  ***************** ************************Reviewer 0EF1*************************************
  
"Novelty/Originality": “Although some of the architectures are new, this is an extension of previous approaches to an existing task -- therefore the paper is not opening up a new direction and might not become seminal. Nevertheless, it establishes a new strong baseline.”

*Response*: We respectfully disagree with this statement, and as mentioned in our response to reviewer "OC1E", this study is novel and different from the previous works in this area. The proposed deliberation system has not been used in any VC-ASR or similar problems such as lip-reading. The proposed deliberation system opens up a feasible way to leverage visual information for the existing audio-only ASR engines. There are also many directions to explore that would reveal more benefits for such a system. Few interesting directions to mention would be applying the same model where the lip-reading information is available, fine-tuning the visual feature extractor model to provide a more accurate visual context, and examining the proposed approach where the audio modality is distorted due to environmental/channel noises. We will mention these examples in the camera-ready version to make the contributions of the paper stand out. 



“Technical Correctness”: “An approach like this involves a number of sub-components, which would be very difficult to evaluate without access to a recipe implementation. But, from my reading, the approaches seem to be correct.”

*Response*: To the best of our knowledge, we have provided all the details of the features and systems used in this study, if the reviewer can mention any specific details that are missing, we can definitely add them in the camera-ready version.
 





“Experimental Validation”:
“Comment1”: “Overall the paper is systematic and careful in its experimentation. 
One criticism is that the paper performs several experiments on the test data. It could maybe have been useful to first do a wide set of experiments on development data, and then only report test results for a smaller subset of the models.
”
*Response*:  As the reviewer acknowledged, we have been careful about the experiments to have an unbiased comparison between the models. We have already considered the reviewer's concern in this study;  in the experiments, the system selection is performed based on the development set, and the reported systems have a consistent performance on development and test sets.   



“*Comment2”: “- Section 4.2: "in Table 1, for the clean audio data, ... the multi-stream architecture ... WER is improved from 17.77\% -> 16.7\%". Should the last number be 17.16\%? If this is not the case, then further clarification is required in this paragraph.
- The qualitative examples in Figure 3 are very useful.”

*Response*: Thanks for the comment. That was a typo, but the performance was correctly reported in Table 1, we will change it to “17.77\% -> 17.16\%” in the camera-ready version. We thank the reviewer for bringing it to our attention.



“Comment3”: “- At first, the improved performance from the deliberation model seemed surprising to me. But then Section 3 clarified this: "... this model introduces a flexible way to leverage the visual information on top of an existing audio-only model that can be trained with a large amount of data." But, from the experiments, it does not seem like the audio component of the deliberation model is actually trained on more data? Are the advantages of the deliberation model, as outlined in the section with that paragraph, actually shown?”

 *Response*: Even though in the deliberation model, the audio-only component can benefit from training with a large amount of audio-only data, but in this study, to have a fair comparison with the previous works, we have only used the HOW2 dataset to train all the models. However, as demonstrated by the detailed experiments, the superiority of the deliberation model is attributed to a more effective architecture to leverage the visual context and the ability of the deliberation model to ground the hypotheses to the visual features. 



“*Clarity of Presentation*”:  “The paper is generally well-written and clear. The following minor comments:

- Minor issue: The word "polish" is used in a number of places to refer to the postprocessing on the N-best lists. This is somewhat informal; could maybe rather use e.g. "refine"?
- "Since speech modality" -> "Since the speech modality"
- "S2S model.(c)" -> "S2S model. (c)"
- Recommend moving Tables 3 and 4 to the bottom of the column, so that the paragraphs aren't split.”

*Response*: We thank the reviewers for bringing these to our attention. We will apply these changes to the camera-ready version. 



“Reference to Prior Work”: “In general I think the references are sufficient. There are work on speech in the context of stationary images which can maybe be mentioned, since they precede some of the mentioned approaches (e.g. the method of joint audio-visual embedding of Harwath et al. came before that of Miech et al.).
https://arxiv.org/abs/1701.07481
https://arxiv.org/abs/1710.01949
https://arxiv.org/abs/1804.01452
”

*Response*: Thanks for pointing out these papers. We will include them in the literature review section.




“Additional comments to author(s)”: “- "In our experiments, we observed that the VC-ASR models trained with video-level visual features were always superior to ones trained with utterance-level visual-feature." Do you think this could potentially be because of a "misalignment" between the speech and the visual context, where e.g. the narrator talks about an object which only then appears somewhat later in the video (i.e. not in the same video frames where the speech occurs)?” 

*Response*: Based on our observations, for some utterances, there is an inherent misalignment between speech and visual context. In addition to that, a wider visual context provides more correlated information and benefits the model more. 




“Comment”: “- It seems like the advantages of the deliberation model (and it's visually grounded hypotheses variant) is that it can take advantage of external (text/audio/vision) resources better than the multi-stream model. Could a language model, trained on large amounts of external text, be easily integrated and was this considered?”

*Response*: In this study, we have not investigated integrating a large language model in the deliberation model, but it would be an interesting direction for future studies. 





****************************************************** Reviewer 0FE6*************************************


“Justification of Novelty/Originality Score”: “The cool thing about the proposed method is that it can be used with existing N-Best audio ASR systems and thus yields some modularity.”

*Response*: Thanks for your comment. 



“Experimental Validation”:   “The masking scenario in the evaluation is very questionable for the reviewer and a major issue. The selection of which words can be masked is based on high values in the word embedding similarity matrix, and thus are words that the visual model is good at recognizing in. This seems very handcrafted to enhance the visual model performance and is far from any realistic scenario, where random words might get lost. When random words are droppen in the data the audio-only model will be better in reestimating them just by using its internal language knowledge (as it already does, shown by the RR for Audio-Only in Table 2). Stating a 59\% relative improvement in recovery rate of the proposed method against the audio-only model thus is NOT a fair comparison, as words are selected for masking that the visual model has a benifit and presumably these task-specifig words are harder for the audio-only model. A simple evaluation of different SNR levels in the audio might be far more realistic.”

*Response*: Firstly, the proposed systems have achieved a significant improvement for the clean audio scenario, and the masking scenario in an additional setting. For the masking scenario, we have followed the literature in VC-ASR [2,3] and VC-translation [4] by choosing words that are highly correlated with the visual feature. In this study, the main motivation for the masking scenario was to examine how well the different proposed VC-ASR models can leverage the visual information to recognize the masked words that are highly correlated with the visual features. We agree with the reviewer that real scenarios can be different and challenging. We have also not claimed that the improvements for the masking scenarios could be generalized to real scenarios.We have already clearly mentioned how we have chosen the masked words in the paper, but to address the reviewer's comments we will clarify it in other parts of the paper too. 



"Clarity of Presentation"
"Comment1": "The Figures in the paper have many issues. In Fig. 1 there are no labels on the axes which makes it difficult to get the whole point of the Figure. What is really shown there? Is it the word embedding values over a time axis? if so please clarify what is actually shown in the underlying video. Maybe show some exemplary image, so one can grasp why 'paper' and 'foam' have so high values."

*Response*: Thanks for your comments. We think that Fig. 1 is well captioned, and it illustrates how each word is correlated with particular frames in the video. However, we agree that adding more detail such as exemplary images would make the figure easier to understand. We will apply the changes to the camera-ready version.




"Comment2": "Fig. 2 has presumably some errors and a lot of visual issues. E.g., for the Multi-Stream model in Fig 2(a): Nothing goes into the decoder, the white font on the yellow 'atten' blocks is unreadable, the [50,512] vector (presumably dimensions) is a label and should NOT be in the signal path (also in Fig 2(b)). Overall parts of the Figure are not refered to in the text and vice Versa (what is y_d and where are the concat or gating mechanisms). Also the visualization in Fig. 2(c) is hard to understand. Maybe use the same terms as in Formulas (3),(4), and (5) to help what is actually going on in this approach."

*Response*: Thanks for the suggestions. In these figures, we have focused on illustrating the proposed approaches and ignored some details of the convectional seq-to-seq models. We will apply some changes to the figures to address all the reviewer's comments, such as using the same terms as the ones used in the equations.


 
[1] Ozan Caglayan, Ramon Sanabria, Shruti Palaskar, Loic Barraul, and Florian Metze, “Multimodal grounding for sequenceto-sequence speech recognition,” in ICASSP 2019-2019 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP). IEEE, 2019, pp. 8648–8652.
[2]. Tejas Srinivasan, Ramon Sanabria, and Florian Metze, “Analyzing utility of visual context in multimodal speech recognition under noisy conditions,” How2 Workshop, ICML 2019.
[3]. Tejas Srinivasan, Ramon Sanabria, and Florian Metze, “Looking enhances listening: Recovering missing speech using images,” in ICASSP 2020-2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP). IEEE, 2020, pp. 6304–6308.
[4]. Ozan Caglayan, Pranava Madhyastha, Lucia Specia, and Lo¨ıc Barrault, “Probing the need for visual context in multimodal machine translation,” NAACL-HLT 2019.



